An Exploration of the Heterogeneous Unsourced MAC

The unsourced MAC model was originally introduced to study the communication scenario in which a number of devices with low-complexity and low-energy wish to upload their respective messages to a base station. In the original problem formulation, all devices communicate using the same information rate. This may be very inefficient in certain wireless situations with varied channel conditions, power budgets, and payload requirements at the devices. This paper extends the original problem setting so as to allow for such variability. More specifically, we consider the scenario in which devices are clustered into two classes, possibly with different SNR levels or distinct payload requirements. In the cluster with higher power,devices transmit using a two-layer superposition modulation. In the cluster with lower energy, users transmit with the same base constellation as in the high power cluster. Within each layer, devices employ the same codebook. At the receiver, signal groupings are recovered using Approximate Message Passing(AMP), and proceeding from the high to the low power levels using successive interference cancellation (SIC). This layered architecture is implemented using Coded Compressed Sensing(CCS) within every grouping. An outer tree code is employed to stitch fragments together across times and layers, as needed.This pragmatic approach to heterogeneous CCS is validated numerically and design guidelines are identified.

==> Simulation_figures.tex <==
\begin{figure}
\begin{tikzpicture}
\definecolor{mycolor1}{rgb}{0.63529,0.07843,0.18431}%
\definecolor{mycolor2}{rgb}{0.00000,0.44706,0.74118}%
\definecolor{mycolor3}{rgb}{0.00000,0.49804,0.00000}%
\definecolor{mycolor4}{rgb}{0.87059,0.49020,0.00000}%
\definecolor{mycolor5}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor6}{rgb}{0.74902,0.00000,0.74902}%

\begin{axis}[%
font=\small,
width=7cm,
height=5.5cm,
scale only axis,
every outer x axis line/.append style={white!15!black},
every x tick label/.append style={font=\color{white!15!black}},
xmin=22,
xmax=34,
xtick = {22,24,...,34},
xlabel={SNR(dB)},
xmajorgrids,
every outer y axis line/.append style={white!15!black},
every y tick label/.append style={font=\color{white!15!black}},
ymin=0.13,
ymax=0.24,
ytick = {0.1,0.13,...,0.24},
ylabel={$R_{tot}$},
ymajorgrids,
legend style={at={(0,1)},anchor=north west, draw=black,fill=white,legend cell align=left}
]



\addplot [color=mycolor2,densely dotted,line width=2.0pt,mark size=1.4pt,mark=o, mark options={solid}]
  table[row sep=crcr]{
23 0.15 \\
24 0.17 \\
25 0.19 \\
26 0.21 \\
27 0.21 \\
28 0.21 \\
29 0.22 \\
30 0.22 \\
31 0.22 \\
32 0.23 \\
33 0.23 \\
};
\addlegendentry{Two layers};


\end{axis}

\end{tikzpicture}
\caption{Simulation results of the best possible sum-rates of two layers given total input power. The per-user error probability constraint here is 5\%.}
\end{figure}
